Maximum likelihood multiple imputation: Faster imputations and consistent standard errors without posterior draws

Multiple imputation (MI) is a method for repairing and analyzing data with missing values. MI replaces missing values with a sample of random values drawn from an imputation model. The most popular form of MI, which we call posterior draw multiple imputation (PDMI), draws the parameters of the imputation model from a Bayesian posterior distribution. An alternative, which we call maximum likelihood multiple imputation (MLMI), estimates the parameters of the imputation model using maximum likelihood (or equivalent). Compared to PDMI, MLMI is less computationally intensive, faster, and yields slightly more efficient point estimates. A past barrier to using MLMI was the difficulty of estimating the standard errors of MLMI point estimates. We derive, implement, and evaluate three consistent standard error formulas: (1) one combines variances within and between the imputed datasets, (2) one uses the score function, and (3) one uses the bootstrap to estimate variance components due to sampling and imputation. Formula (1) modifies for MLMI a formula that has long been used under PDMI, while formulas (2) and (3) can be used without modification under either PDMI or MLMI. We have implemented MLMI and the standard error estimators in the mlmi and bootImpute packages for R.

==> outtakes.tex <==
\begin{subtable}{\textwidth}
            \centering
            \caption{Mean length of score based (SB) nominal 95\% CIs for $\beta_{X.Y}$ (with \% departure from 95\% coverage).}
\begin{tabular}{ c c c   c c c   c}
\hline
\multicolumn{2}{c}{Missing}& &\multicolumn{2}{c}{SB $(\alpha_{X.Y}, \beta_{X.Y}, \sigma^{2}_{X.Y})$}  &\multicolumn{2}{c}{SB $(\alpha_{X.Y}, \beta_{X.Y}, \sigma^{2}_{X.Y},\mu_{Y},\sigma^{2}_{Y})$} \\
\cline{1-2} \cline{4-7}
\% & Pattern & Imputations &PDMI &MLMI &PDMI &MLMI \\
\hline
25 & MCAR & 10 & 0.17 (0.6) & 0.17 (0.5) & 0.17 (0.8) & 0.17
(0.7)\tabularnewline
 &  & 50 & 0.17 (0.7) & 0.17 (0.6) & 0.17 (0.8) & 0.17
(0.9)\tabularnewline
 &  & 200 & 0.17 (0.3) & 0.17 (0.2) & 0.17 (0.5) & 0.17
(0.4)\tabularnewline
 & MAR & 10 & 0.17 (-0.2) & 0.17 (-0.1) & 0.17 (0.1) & 0.17
(0.2)\tabularnewline
 &  & 50 & 0.17 (0.1) & 0.17 (0.0) & 0.17 (0.3) & 0.17
(0.3)\tabularnewline
 &  & 200 & 0.17 (0.1) & 0.17 (0.0) & 0.17 (0.3) & 0.17
(0.3)\tabularnewline
50 & MCAR & 10 & 0.20 (0.2) & 0.20 (0.0) & 0.21 (0.5) & 0.20
(0.3)\tabularnewline
 &  & 50 & 0.20 (0.1) & 0.20 (0.0) & 0.20 (0.4) & 0.20
(0.2)\tabularnewline
 &  & 200 & 0.20 (0.5) & 0.20 (0.5) & 0.20 (0.8) & 0.20
(0.8)\tabularnewline
 & MAR & 10 & 0.21 (-1.4) & 0.20 (-1.2) & 0.22 (0.8) & 0.22
(0.6)\tabularnewline
 &  & 50 & 0.20 (-1.3) & 0.20 (-1.5) & 0.22 (0.6) & 0.22
(0.5)\tabularnewline
 &  & 200 & 0.20 (-1.0) & 0.20 (-1.2) & 0.22 (0.9) & 0.21
(0.5)\tabularnewline
\hline
\end{tabular}
\end{subtable}




\begin{subtable}{\textwidth}
            \centering
            \caption{Mean length of nominal 95\% CIs for $\beta_{X.Y}$ (with \% departure from 95\% coverage) using within between (WB) method applied to different subsets of the parameters.}
\begin{tabular}{ c c c   c c c   c}
\hline
\multicolumn{2}{c}{Missing}& &  &\multicolumn{3}{c}{MLMI} \\
\cline{1-2} \cline{5-7} 
 &  & & & & $(\alpha_{X.Y}, \beta_{X.Y}, $ & $(\alpha_{X.Y}, \beta_{X.Y},$ \\
\% & Pattern & Imputations &PDMI &$(\alpha_{X.Y}, \beta_{X.Y})$ & $\sigma^{2}_{X.Y})$ & $ \sigma^{2}_{X.Y},\mu_{Y},\sigma^{2}_{Y})$ \\
\hline
25 & MCAR & 10 & 0.17 (0.3) & 0.17 (0.9) & 0.17 (1.0) & 0.18
(1.2)\tabularnewline
 &  & 50 & 0.17 (0.5) & 0.17 (0.3) & 0.17 (0.5) & 0.17
(0.5)\tabularnewline
 &  & 200 & 0.17 (0.0) & 0.17 (-0.2) & 0.17 (0.0) & 0.17
(0.1)\tabularnewline
 & MAR & 10 & 0.17 (-0.3) & 0.17 (0.1) & 0.18 (0.3) & 0.18
(0.4)\tabularnewline
 &  &  & 0.17 (-0.1) & 0.17 (-0.1) & 0.17 (0.1) & 0.17
(0.3)\tabularnewline
 &  & 200 & 0.17 (0.1) & 0.17 (-0.4) & 0.17 (-0.2) & 0.17
(0.0)\tabularnewline
50 & MCAR & 10 & 0.20 (0.0) & 0.20 (-0.2) & 0.21 (0.2) & 0.21
(0.7)\tabularnewline
 &  &  & 0.20 (0.1) & 0.19 (-1.1) & 0.20 (0.0) & 0.21
(0.4)\tabularnewline
 &  & 200 & 0.20 (0.4) & 0.19 (-0.9) & 0.20 (0.2) & 0.20
(0.5)\tabularnewline
 & MAR & 10 & 0.22 (0.0) & 0.20 (-1.7) & 0.21 (-1.4) & 0.21
(-0.9)\tabularnewline
 &  &  & 0.21 (0.3) & 0.19 (-2.8) & 0.20 (-1.1) & 0.22
(0.2)\tabularnewline
 &  & 200 & 0.21 (0.5) & 0.19 (-2.9) & 0.20 (-1.2) & 0.22
(0.5)\tabularnewline
\hline
\end{tabular}
\end{subtable}

\begin{subtable}{\textwidth}
            \centering
            \caption{Mean length of nominal 95\% CIs for $\beta_{X.Y}$ (with \% departure from 95\% coverage) using bootstrapped MI.}
\begin{tabular}{ c c c   c c }
\hline
\% & Pattern & Imputations & BPDMI & BMLMI \\
\hline
25 & MCAR & 50 & 0.18 (0.1) & 0.18 (0.5)\tabularnewline
 &  & 200 & 0.17 (-0.2) & 0.17 (-0.1)\tabularnewline
 & MAR & 50 & 0.18 (-0.2) & 0.18 (-0.4)\tabularnewline
 &  & 200 & 0.17 (-0.3) & 0.17 (-0.2)\tabularnewline
50 & MCAR & 50 & 0.21 (-0.2) & 0.21 (-0.4)\tabularnewline
 &  & 200 & 0.20 (0.3) & 0.20 (-0.1)\tabularnewline
 & MAR & 50 & 0.23 (0.3) & 0.23 (0.0)\tabularnewline
 &  & 200 & 0.21 (0.2) & 0.21 (0.1)\tabularnewline
\hline
\end{tabular}
\end{subtable}

Tables \ref{mcsCatVars} and \ref{mcsCtsVars} summarize the categorical and continuous variables in the data. The percentage of missing values varied from 0.013\% (number of siblings) to 15.8\% (family income).

\begin{table}[ht]
\caption{Distribution of categorical variables in Millenium Cohort Study data} 
\label{mcsCatVars}
\centering
\begin{tabular}{llll}
  \hline
Variable & Level & Number & \% \\ 
  \hline
Marital status & Not married & 5030 & 31.8 \\ 
   & Married & 9954 & 63 \\ 
   & Missing & 824 & 5.21 \\ 
  Housing tenure & Owned & 10098 & 63.9 \\ 
   & Rented & 5021 & 31.8 \\ 
   & Other & 542 & 3.43 \\ 
   & Missing & 147 & 0.93 \\ 
  History of hearing loss & Yes & 690 & 4.36 \\ 
   & No & 14870 & 94.1 \\ 
   & Missing & 248 & 1.57 \\ 
  Ethnicity & White & 12871 & 81.4 \\ 
   & Non-white & 2184 & 13.8 \\ 
   & Missing & 753 & 4.76 \\ 
  Respondent in work & In work & 8025 & 50.8 \\ 
   & Not in work & 7635 & 48.3 \\ 
   & Missing & 148 & 0.936 \\ 
  No. siblings & 0 & 4130 & 26.1 \\ 
   & 1 & 6973 & 44.1 \\ 
   & 2 & 3024 & 19.1 \\ 
   & 3 or more & 1679 & 10.6 \\ 
   & Missing & 2 & 0.0127 \\ 
   \hline
\end{tabular}
\end{table}

\begin{table}[ht]
\caption{Distribution of continuous variables in Millenium Cohort Study data}
\label{mcsCtsVars}
\centering
\begin{tabular}{lll}
  \hline
Variable & Mean (SD) & No. missing (\%) \\ 
  \hline
Bracken score & 103.4 (16.3) & 1769 (11.2) \\ 
  Family income code & 10 (3.9) & 2501 (15.8) \\ 
  Respondent age & 31.9 (6) & 21 (0.133) \\ 
   \hline
\end{tabular}
\end{table}

Different variance formulas make different assumptions about the analysis and imputation models, and violations of these assumptions can affect performance. The bootstrap assumes relatively little and can produce asymptotically consistent variance estimates even when the analysis and imputation models are different and misspecified. Bootstrap CIs may have poor coverage if point estimates are biased, but the bootstrap variance estimates themselves will be asymptotically consistent.

The WB formulas assume more. Under PDMI, the WB formula assumes that the analysis and imputation models are correctly specified and "congenial" in the sense that the imputation model includes all the variables in the analysis model and does not constrain the relationships among those variables in ways that the analysis model does not (Meng 1994). If the imputation model includes more variables than the analysis model, then the WB formula may overestimate $V_{MI}$, producing "conservative" CIs which are wider than necessary and have higher than nominal coverage (Meng 1994).

Under MLMI, the WB formula assumes even more, as does the SB formula (under both MLMI and PDMI). These formulas are derived in part from \eqref{V_MLMI} and \eqref{V_PDMI}, which assume that the imputation and analysis models are not just correct but the same (Wang \& Robins 1998). When that assumption is met (Table \ref{tab:Y_on_X}), SB and WB CIs have good coverage even when the fraction of missing information is large. When that assumption is violated (Table \ref{tab:X_on_Y}), SB and WB CIs still have good coverage in simulations where the fraction of missing information is small to moderate ($\gamma_{mis}<.3$) --- as it is in many applied datasets. When the fraction of missing information is larger, then SB and WB CIs can be too short, and again it is better to use the bootstrap.

So when you use the PDMI WB formula, you don't have to worry about whether you are including 

When you use the PDMI WB formula, it does not matter whether you include every component of $\theta$. You can omit parameters from the joint model that underlies the imputation and analysis model. YOu can It doesn't even matter whether $theta $

Therefore adding parameters to the $\theta$ vector has no effect on the standard 

can be used in either matrix or scalar form. If you have a vector of parameter estimates ${\widehat{\theta}}_{PDMI,WB}$, you can apply the WB formula to the matrices ${\widehat{W}}_{PDMI}$ and ${\widehat{B}}_{PDMI}$, and get a matrix ${\widehat{V}}_{PDMI,WB}$ whose diagonal contains squared standard errors for each component of ${\widehat{\theta}}_{PDMI,WB}$. Alternatively, you can select scalar components of ${\widehat{\theta}}_{PDMI,WB}$, apply the WB formula to the corresponding diagonal components of ${\widehat{W}}_{PDMI}$ and ${\widehat{B}}_{PDMI}$, and get the same standard errors. The matrix and scalar approaches are equivalent because the WB formula only 

This is a nice property because in some applications, software may not provide the full matrix  ${\widehat{W}}_{PDMI}$. Instead, it may only provide the standard errors whose squares line the diagonal of ${\widehat{W}}_{PDMI}$. In addition, the user might not want a standard error for every component of ${\widehat{\theta}}_{PDMI,WB}$, but only for certain statistics such as the means of key variables. It is comforting to know that the scalar WB formula still works when applied only to a submatrix or matrix diagonal .

Importantly WB variance estimates can still be consistent in this case provided the imputation and analysis models are congenial (Meng 1994). Under uncongeniality, WB variance estimates can be biased upwards or downwards, although some (Meng 1994) have argued that typically it will be biased upwards, leading to conservative inferences. Even in such settings, it would be better to have variance estimates that were consistent, and confidence intervals that have exactly nominal coverage.

In practice, though, the analysis model is often different from the imputation model, and none of the variance estimators discussed so far is guaranteed consistent. Under PDMI, when the models are ``congenial''---i.e., the assumptions of the analysis model do not contradict the assumptions of the imputation models---then WB variance estimates are ``conservative'' in the sense that any bias in the variance estimate is positive and confidence intervals have at least nominal coverage (Meng 1994). But of course it would be better to have variance estimates that were consistent and unbiased, and confidence intervals that have exactly nominal coverage.

Could  we limit calculations to the $2\times2$ or $3\times3$ matrix describing the covariances among the two or three estimated parameters of the regression -- e.g., $\widehat{\alpha}_{X.Y},\widehat{\beta}_{X.Y}$ and possibly $\widehat{\sigma^2}_{X.Y}$ for the regression of $X$ on $Y$? Or must we use the the full $5\times5$ matrix describing the covariances among the five parameter estimates describing the bivariate normal distibution of $(X,Y)$? \footnote{There are several equivalent ways to define the five parameters of the bivariate normal distribution. When interested in the regression of $X$ on $Y$, we used the parameters of that regression ($\alpha_{X.Y},\beta_{X.Y},\sigma_{Y.X}^2)$ and the parameters $(\mu_X,\sigma_X^2)$ of the marginal distribution of $X$. If interested in regression of $Y$ on $X$, though, we could use the parameters of that regression ($\alpha_{X.Y},\beta_{X.Y},\sigma_{Y.X}^2)$ and the parameters $(\mu_X,\sigma_X^2)$ of the marginal distribution of $Y$.} In our initial simulation, we used a 3x3 matrix for the SB matrix calculations in \ref{section:SB_variance_estimation} and a 2x2 matrix for the MLMI WB matrix calculations in \ref{subsection:MLMI_WB}. In a followup simulation, we used the full 5x5 covariance matrix. 

\section{Block-wise application of WB MLMI variance estimator}
\label{appendix:block_diagonal}
The MLMI WB variance estimator of equation \eqref{V_MLMI_WB} is equal to (suppressing the MLMI subscripts)
\begin{eqnarray*}
\widehat{W} (I - \widehat{W}^{-1} \widehat{B})^{-1} + \frac{1}{M} \widehat{B}
\end{eqnarray*}
It is justified from the results of Wang and Robins (1998) when the imputation and analysis models are the same joint model for the full data vector. In this appendix we consider under what alternative situations the estimator remains valid when this is not the case.

Let $f(Y|\theta_{1},\theta_{2})$ denote a joint model for the complete data vector, such that 
\begin{eqnarray*}
f(Y|\theta_{1},\theta_{2})=f_{1}(Y|\theta_{1}) f_{2}(Y|\theta_{2})
\end{eqnarray*}
and with $\theta_{1}$ and $\theta_{2}$ distinct parameters (the parameter space is the product of the individual parameter spaces). Suppose further that $\theta_{1}$ is the parameter of interest. Then it follows (Section 7.1 of Little and Rubin (2002)) that the complete data variance $V_{com}$ covariance matrix for $(\theta_{1},\theta_{2})$ is block diagonal, and thus so is our estimate of this, $\widehat{W}$. Thus we can write
\begin{eqnarray*}
\widehat{W} = \begin{pmatrix} \widehat{W}_{1} & 0 \\ 0 &  \widehat{W}_{2} \end{pmatrix}
\end{eqnarray*}
Then since $\widehat{W}$ is block diagonal we have
\begin{eqnarray*}
\widehat{W}^{-1} = \begin{pmatrix} \widehat{W}^{-1}_{1} & 0 \\ 0 & \widehat{W}^{-1}_{2} \end{pmatrix}
\end{eqnarray*}
is also block diagonal. Next we let 
\begin{eqnarray*}
\widehat{B} = \begin{pmatrix} \widehat{B}_{11} & \widehat{B}_{12} \\ \widehat{B}^{T}_{12} & \widehat{B}_{22} \end{pmatrix}
\end{eqnarray*}
be the between imputation covariance matrix, with blocks corresponding to $\theta_{1}$ and $\theta_{2}$. Then further matrix algebra then shows that the top left block in $\widehat{W} (I - \widehat{W}^{-1} \widehat{B})^{-1}$, which contributes to the variance of the estimate of $\theta_{1}$ is equal to
\begin{eqnarray}
\widehat{W}_{1} \left[ I - \widehat{W}^{-1}_{1} \widehat{B}_{11} - \widehat{W}^{-1}_{1} \widehat{B}_{12}(I - \widehat{W}^{-1}_{2} \widehat{B}_{22})^{-1} \widehat{W}^{-1}_{2} \widehat{B}^{T}_{12} \right ]^{-1}
\label{mlmiWBTheta1Full}
\end{eqnarray}
where $I$ denotes the identity matrix. If $\widehat{B}_{12}=0$, then this reduces to 
\begin{eqnarray}
\widehat{W}_{1} \left( I - \widehat{W}^{-1}_{1} \widehat{B}_{11} \right )^{-1}
\label{mlmiWBTheta1BlockWise}
\end{eqnarray}
which is what would be obtained were the variance formula \eqref{V_MLMI_WB} to be applied only to $\theta_{1}$. Thus application of the variance formula to only $\theta_{1}$ is justified if $\widehat{B}_{12}=0$. One situation where this occurs is if the between imputation variance of estimates of $\theta_{2}$ is zero. This in turn occurs if the component of the joint density $f(Y|\theta_{2})$ is unaffected by missing data. An example is the setting of our first simulation study, where the parameter of interest $\theta_{1}$ corresponds to the parameters in the model for $f(Y|X)$, only $Y$ has missing values, and $\theta_{2}$ corresponds to parameters indexing a model for the marginal distribution of $X$.

When $\theta_{1}$ is a scalar, it is clear from comparison of equation \eqref{mlmiWBTheta1Full} with equation \eqref{mlmiWBTheta1BlockWise} that applying variance formula \eqref{V_MLMI_WB} only to $\theta_{1}$ will result in an underestimation of its variance. When $\theta_{1}$ is a vector, SOME FURTHER ARGUMENTS I SUSPECT WILL SHOW THAT ONE AGAIN UNDERESTIMATES VARIANCE IN THE SENSE THAT EQUATION \eqref{mlmiWBTheta1Full} MINUS EQUATION \eqref{mlmiWBTheta1BlockWise} IS POSITIVE DEFINITE.

Why do the SB and MLMI WB formulas require that matrix calculations include all five parameters? As discussed in section \ref{section:matrix_vs_scalar}, the formulas involve matrix multiplication, so that off-diagonal elements (covariances) of the matrices being multiplied can affect the diagonal elements (variances) of the final result. That is, we must estimate the whole 5x5 covariance matrix in order to estimate any of the variances consistently.

By contrast, the bootstrap and PDMI WB formulas do not require that we use the 5x5 covariance matrix. They will provide the same, consistent estimates whether we use the 5x5 matrix or just the $2\times2$ submatrix describing the distribution of ($\widehat{\alpha}_{X.Y},\widehat{\beta}_{X.Y}$). That's because the bootstrap and PDMI WB formulas only involve addition. They can be used in scalar form, and if they are used in matrix form, the off-diagonal elements of the component matrices (covariances) cannot affect the diagonal elements of the sum (variances).

Why didn't this come up when we regressed the $Y$ on $X$? In that situation, the estimated regression slope and intercept ($\widehat{\alpha}_{Y.X},\widehat{\beta}_{Y.X}$) were independent of the other parameter estimates. In the full 5x5 covariance matrix, the off-diagonal terms relating ($\widehat{\alpha}_{Y.X},\widehat{\beta}_{Y.X}$) to the other estimates were zero and could be neglected. The same is not true when we regress $X$ on $Y$. For details, see Appendix \label{appendix:block_diagonal}.

\bibitem{Allison2000} Allison, P. D. (2000, February 23). The \%miss macro, version 1.05. Retrieved March 15, 2012, from http://www.ssc.upenn.edu/$\sim$allison/miss.sas

\bibitem{Andridge2015}Andridge, R., \& Thompson, K. J. (2015). Assessing nonresponse bias in a business survey: Proxy pattern-mixture analysis for skewed data. The Annals of Applied Statistics, 9(4), 2237–2265. https://doi.org/10.1214/15-AOAS878

\bibitem{Bodner2008}Bodner, T. E. (2008). What Improves with Increased Missing Data Imputations? Structural Equation Modeling, 15(4), 651–675.

\bibitem{Buuren2011}Van Buuren, Stef and Karin Groothuis-Oudshoorn. (2011). mice: Multivariate Imputation by Chained Equations in R. Journal of Statistical Software. 45(3).


\bibitem{Efron1994} Efron, B. (1994). Missing Data, Imputation, and the Bootstrap. Journal of the American Statistical Association, 89(426), 463--475. http://doi.org/10.2307/2290846.


\bibitem{Honaker1998} Honaker, J., Joseph, A., King, G., \& Scheve, K. (1998). Amelia: A Program for Missing Data.


\bibitem{Hu2013}Hu, J., Mitra, R., and Reiter, J. P. (2013), Are Independent Draws Necessary for Multiple Imputation?, The American Statistician, 67, 143 - 149.



\bibitem{LittleRubin1989}Little, R. J. A., & Rubin, D. B. (1989). The Analysis of Social Science Data with Missing Values. Sociological Methods & Research, 18(2-3), 292 –326. http://doi.org/10.1177/0049124189018002004

\bibitem{Quezada2017} Quezada-Hofflinger, Alvaro and von Hippel, Paul T., The Response to High Stakes Testing in Chile 2005-2013: Legitimate and Illegitimate Ways to Raise Test Scores (January 25, 2017). Available at SSRN: https://ssrn.com/abstract=2906552


\bibitem{Raghunathan2001} Raghunathan, T. E., Lepkowski, J. M., Van Hoewyk, J., \& Solenberger, P. W. (2001). A Multivariate Technique for Multiply Imputing Missing Values Using a Sequence of Regression Models. Survey Methodology, 27(1), 85--95.


\bibitem{vH2007} von Hippel, P. T. (2007). Regression With Missing Ys: An Improved Strategy For Analyzing Multiply Imputed Data. Sociological Methodology, 37, 83–117.
